ANATAR: AN Automated Tool for higher-order Amplitude geneRation

We present a new Mathematica package that provides a platform to perform multi-loop computations. ANATAR integrates several existing tools designed for higher-order computations. In particular, it uses QGRAF to generate Feynman diagrams and relies on FORM to perform the Dirac and colour algebras. This makes it very efficient without compromising user-friendliness and flexibility. In addition, ANATAR is equipped with functionalities to manipulate the generated amplitudes and to extract scalar form factors. The resulting expressions can be mapped to integral families that can subsequently be reduced to master integrals via dedicated interfaces to codes for integration-by-parts reduction. Support for large classes of BSM models with the same gauge group as the SM is provided, and in particular, ANATAR is optimised for computations in effective field theories. We review and introduce the main functionalities of ANATAR and illustrate its use for phenomenological applications.

==> intro.tex <==
% !TEX root = anatar.tex


Scattering amplitudes are arguably among the most important objects in many areas of modern high-energy physics.  





